A New Confidence Interval for Odds Ratio

We consider the problem of interval estimation of the odds ratio. An asymptotic confidence interval is widely applied in medical research. Unfortunately that confidence interval has a poor coverage probability: it is significantly smaller than the nominal confidence level. In this paper a new confidence interval is proposed. The construction needs only information on sample sizes and sample odds ratio. The coverage probability of the proposed confidence interval is at least the nominal confidence level.

==> Pokrycie_moje.tex <==
%r_teor	Poziom_moj
0.1	0.974987601
0.15	0.974707427
0.2	0.97341666
0.25	0.975335772
0.3	0.975073767
0.35	0.975099587
0.4	0.975960361
0.45	0.975338152
0.5	0.975508464
0.55	0.974998357
0.6	0.975991279
0.65	0.975147667
0.7	0.975098489
0.75	0.975086397
0.8	0.975127458
0.85	0.950236524
0.9	0.950285205
0.95	0.95033952
1	0.95024915
1.05	0.950342123
1.1	0.950639507
1.15	0.950633275
1.2	0.950269467
1.25	0.975127458
1.3	0.975575126
1.35	0.97529973
1.4	0.975969821
1.45	0.975253266
1.5	0.975074636
1.55	0.975105909
1.6	0.975161173
1.65	0.975795525
1.7	0.97636154
1.75	0.975104236
1.8	0.975223062
1.85	0.975313217
1.9	0.975824112
1.95	0.97512715
2	0.975508464


==> Pokrycie_std.tex <==
%r_teor	Poziom_std
0.1	0.8313239
0.15	0.8617767
0.2	0.8792762
0.25	0.8890853
0.3	0.8959760
0.35	0.9003521
0.4	0.9042889
0.45	0.9071868
0.5	0.9073538
0.55	0.9102443
0.6	0.9109428
0.65	0.9127746
0.7	0.9135993
0.75	0.9147535
0.8	0.9143139
0.85	0.9149293
0.9	0.9140068
0.95	0.9139714
1	0.9154840
1.05	0.9138629
1.1	0.9150363
1.15	0.9149839
1.2	0.9140325
1.25	0.9143139
1.3	0.9145431
1.35	0.9140730
1.4	0.9127034
1.45	0.9127548
1.5	0.9130438
1.55	0.9126043
1.6	0.9127003
1.65	0.9114342
1.7	0.9113234
1.75	0.9111424
1.8	0.9096912
1.85	0.9111513
1.9	0.9106043
1.95	0.9101988
2	0.9073538

